Flattened Stirling Permutations

Recall that a Stirling permutation is a permutation on the multiset $\{1,1,2,2,\ldots,n,n\}$ such that any numbers appearing between repeated values of $i$ must be greater than $i$. We call a Stirling permutation ``flattened'' if the leading terms of maximal chains of ascents (called runs) are in weakly increasing order. Our main result establishes a bijection between flattened Stirling permutations and type $B$ set partitions of $\{0,\pm1,\pm2,\ldots,\pm (n-1)\}$, which are known to be enumerated by the Dowling numbers, and we give an independent proof of this fact. We also determine the maximal number of runs for any flattened Stirling permutation, and we enumerate flattened Stirling permutations with a small number of runs or with two runs of equal length. We conclude with some conjectures and generalizations worthy of future investigation.

==> AziasFigure.tex <==
    \begin{tikzpicture}

%Nodes 
\draw[fill] (0,0) circle [radius=0.1];
\node at (0,-.5) {$0|1|2|3$};
\node at (0,-1) {\tiny{\textcolor{blue}{$11223344$}}};

% 1st floor Nodes
\draw[fill] (0,0.7) circle [radius=0.1];
\node at (0,1.5) {$0|1|23$};
\node at (0,1) {\tiny{\textcolor{blue}{$11223443$}}};

\draw[fill] (-1.25,0.7) circle [radius=0.1];
\node at (1.3,1.5) {$0|\Bar{2}1|3$};
\node at (1.25,1) {\tiny{\textcolor{blue}{$11332244$}}};

\draw[fill] (1.25,.7) circle [radius=0.1];
\node at (-1.3,1.5) {$02|1|3$};
\node at (-1.3,1) {\tiny{\textcolor{blue}{$13312244$}}};

\draw[fill] (-2.5,.7) circle [radius=0.1];
\node at (-2.6,1.5) {$0|13|2$};
\node at (-2.55,1) {\tiny{\textcolor{blue}{$11244233$}}};

\draw[fill] (2.5,.7) circle [radius=0.1];
\node at (2.6,1.5) {$03|1|2$};
\node at (2.55,1) {\tiny{\textcolor{blue}{$14412233$}}};

\draw[fill] (-3.5,.7) circle [radius=0.1];
\node at (-3.8,1.5) {$0|12|3$};
\node at (-3.8,1.0) {\tiny{\textcolor{blue}{$11233244$}}};

\draw[fill] (3.5,.7) circle [radius=0.1];
\node at (3.8,1.5) {$0|\Bar{3}1|2$};
\node at (3.8,1) {\tiny{\textcolor{blue}{$11442233$}}};


\draw[fill] (4.8,.7) circle [radius=0.1];
\node at (5,1.5) {$0|1|\Bar{3}2$};
\node at (5,1) {\tiny{\textcolor{blue}{$11224433$}}};

\draw[fill] (-4.8,.7) circle [radius=0.1];
\node at (-5,1.5) {$01|2|3$};
\node at (-5,1) {\tiny{\textcolor{blue}{$12213344$}}};


%2nd base vertices
\draw[fill] (-4.9,2) circle [radius=0.1]; %1
\draw[fill] (-3.8,2) circle [radius=0.1];
\draw[fill] (-2.6,2) circle [radius=0.1]; %3
\draw[fill] (-1.2,2) circle [radius=0.1];
\draw[fill] (0,2) circle [radius=0.1]; %5
\draw[fill] (1.2,2) circle [radius=0.1];
\draw[fill] (2.6,2) circle [radius=0.1]; %7
\draw[fill] (3.8,2) circle [radius=0.1];
\draw[fill] (4.9,2) circle [radius=0.1]; %9
%2nd floor top vertices 
\draw[fill] (-8.9,4.5) circle [radius=0.1]; %1
\draw[fill] (-7.5,4.5) circle [radius=0.1]; 
\draw[fill] (-6.0,4.5) circle [radius=0.1]; %3
\draw[fill] (-4.5,4.5) circle [radius=0.1];
\draw[fill] (-3.0,4.5) circle [radius=0.1]; %5
\draw[fill] (-1.5,4.5) circle [radius=0.1];
\draw[fill] (0,4.5) circle [radius=0.1]; %7
\draw[fill] (1.5,4.5) circle [radius=0.1]; 
\draw[fill] (3.0,4.5) circle [radius=0.1]; %9
\draw[fill] (4.5,4.5) circle [radius=0.1];
\draw[fill] (6.0,4.5) circle [radius=0.1]; %11
\draw[fill] (7.5,4.5) circle [radius=0.1]; 
\draw[fill] (9,4.5) circle [radius=0.1]; %13



%Lines
\draw[thick](0,0)--(0,0.7);
\draw[thick](0,0)--(1.25,.7);
\draw[thick](0,0)--(-1.25,.7);
\draw[thick](0,0)--(-2.5,.7);
\draw[thick](0,0)--(2.5,.7);
\draw[thick](0,0)--(3.5,.7);
\draw[thick](0,0)--(-3.5,.7);
\draw[thick](0,0)--(4.8,.7);
\draw[thick](0,0)--(-4.8,.7);

%\draw[very thick,loosely dotted](-4.9,2)--(-9.0,4.5);
%\draw[very thick,loosely dotted](4.8,2)--(-9.0,4.5);
\draw[very thin](-4.9,2)--(-9.0,4.5);
\draw[very thin](4.8,2)--(-9.0,4.5);

\draw[very thin](-4.9,2)--(-7.5,4.5);
\draw[very thin](-3.8,2)--(-7.5,4.5);
\draw[very thin](-1.2,2)--(-7.5,4.5);
\draw[very thin](1.2,2)--(-7.5,4.5);

\draw[very thin](-4.9,2)--(-6.0,4.5);
\draw[very thin](0,2)--(-6.0,4.5);

\draw[very thin](-3.8,2)--(-4.5,4.5);
\draw[very thin](-2.6,2)--(-4.5,4.5);
\draw[very thin](0,2)--(-4.5,4.5);

%\draw[very thick,loosely dotted](-2.6,2)--(-3.0,4.5);
%\draw[very thick,loosely dotted](-1.2,2)--(-3.0,4.5);
\draw[very thin](-2.6,2)--(-3.0,4.5);
\draw[very thin](-1.2,2)--(-3.0,4.5);

\draw[very thin](-1.2,2)--(-1.5,4.5);
\draw[very thin](0,2)--(-1.5,4.5);
\draw[very thin](2.6,2)--(-1.5,4.5);
\draw[very thin](4.9,2)--(-1.5,4.5);

%\draw[very thick,loosely dotted](-2.6,2)--(0,4.5);
%\draw[very thick,loosely dotted] (1.2,2)--(0,4.5);
%\draw[very thick,loosely dotted](4.9,2)--(0,4.5);
\draw[very thin](-2.6,2)--(0,4.5);
\draw[very thin] (1.2,2)--(0,4.5);
\draw[very thin](4.9,2)--(0,4.5);

\draw[very thin](-1.2,2)--(1.5,4.5);
\draw[very thin](3.8,2)--(1.5,4.5);

\draw[very thin](0,2)--(3.0,4.5);
\draw[very thin](1.2,2)--(3.0,4.5);
\draw[very thin](3.8,2)--(3.0,4.5);

%\draw[very thick,loosely dotted](1.2,2)--(4.5,4.5);
%\draw[very thick,loosely dotted](2.6,2)--(4.5,4.5);
\draw[very thin](1.2,2)--(4.5,4.5);
\draw[very thin](2.6,2)--(4.5,4.5);

\draw[very thin](-4.9,2)--(6.0,4.5);
\draw[very thin](2.6,2)--(6.0,4.5);
\draw[very thin](3.8,2)--(6.0,4.5);

\draw[very thin](-3.8,2)--(7.5,4.5) ;
\draw[very thin](2.6,2)--(7.5,4.5);

\draw[very thin](-3.8,2)--(9,4.5);
\draw[very thin](3.8,2)--(9.0,4.5);
\draw[very thin](4.9,2)--(9.0,4.5);

%3rd floor nodes
\node at (-9.0,5.2) {$01|\Bar{3}2$};
\node at (-9.0,4.82) {\tiny{\textcolor{blue}{$12214433$}}};

\node at (-7.5,5.2) {$012|3$};
\node at (-7.5,4.82) {\tiny{\textcolor{blue}{$12233144$}}};

\node at (-6,5.2) {$01|23$};
\node at (-6,4.82) {\tiny{\textcolor{blue}{$12213443$}}};

\node at (-4.5,5.2) {$0|123$};
\node at (-4.5,4.82) {\tiny{\textcolor{blue}{$11233442$}}};

\node at (-3,5.2) {$02|13$};
\node at (-3,4.82) {\tiny{\textcolor{blue}{$13312442$}}};

\node at (-1.5,5.2) {$023|1$};
\node at (-1.5,4.82) {\tiny{\textcolor{blue}{$13344122$}}};

\node at (0,5.2) {$0|\Bar{2}13$};
\node at (0,4.82) {\tiny{\textcolor{blue}{$11332442$}}}; 

\node at (1.5,5.2) {$02|\Bar{3}1$};
\node at (1.5,4.82) {\tiny{\textcolor{blue}{$13314422$}}}; 

\node at (3,5.2) {$0|\Bar{2}\Bar{3}1$};
\node at (3,4.82) {\tiny{\textcolor{blue}{$11334422$}}}; 

\node at (4.5,5.2) {$03|\Bar{2}1$};
\node at (4.5,4.82) {\tiny{\textcolor{blue}{$14413322$}}};

\node at (6,5.2) {$013|2$};
\node at (6,4.82) {\tiny{\textcolor{blue}{$12244133$}}};

\node at (7.5,5.2) {$03|12$};
\node at (7.5,4.82) {\tiny{\textcolor{blue}{$14412332$}}};

\node at (9,5.2) {$0|\Bar{3}12$};
\node at (9,4.82) {\tiny{\textcolor{blue}{$11442332$}}};

%4th floor node
\node at (0,7.6) {$0123$};
\node at (0,7.2) {\tiny{\textcolor{blue}{$12233441$}}};

%3rd base vertices 
\draw[fill] (0,6.8) circle [radius=0.1]; 

\draw[fill] (-9.0,5.7) circle [radius=0.1]; %1
\draw[fill] (-7.5,5.7) circle [radius=0.1]; 
\draw[fill] (-6.0,5.7) circle [radius=0.1]; %3
\draw[fill] (-4.5,5.7) circle [radius=0.1];
\draw[fill] (-3.0,5.7) circle [radius=0.1]; %5
\draw[fill] (-1.5,5.7) circle [radius=0.1];
\draw[fill] (0,5.7) circle [radius=0.1]; %7
\draw[fill] (1.5,5.7) circle [radius=0.1]; 
\draw[fill] (3.0,5.7) circle [radius=0.1]; %9
\draw[fill] (4.5,5.7) circle [radius=0.1];
\draw[fill] (6.0,5.7) circle [radius=0.1]; %11
\draw[fill] (7.5,5.7) circle [radius=0.1]; 
\draw[fill] (9,5.7) circle [radius=0.1]; %13 

%Lines 
\draw[very thin] (-9.0,5.7)--(0,6.8);
\draw[very thin] (-7.5,5.7)--(0,6.8);
\draw[very thin] (-6.0,5.7)--(0,6.8);
\draw[very thin] (-4.5,5.7)--(0,6.8);
\draw[very thin] (-3.0,5.7)--(0,6.8);
\draw[very thin] (-1.5,5.7)--(0,6.8);
\draw[very thin] (0,5.7)--(0,6.8);
\draw[very thin] (1.5,5.7)--(0,6.8);
\draw[very thin] (3.0,5.7)--(0,6.8);
\draw[very thin] (4.5,5.7)--(0,6.8);
\draw[very thin] (6.0,5.7)--(0,6.8);
\draw[very thin] (7.5,5.7)--(0,6.8);
\draw[very thin] (9,5.7)--(0,6.8);


    \end{tikzpicture}
    
